XR Prototyping of Mixed Reality Visualizations: Compensating Interaction Latency for a Medical Imaging Robot

Researching novel user experiences in medicine is challenging due to limited access to equipment and strict ethical protocols. Extended Reality (XR) simulation technologies offer a cost- and time-efficient solution for developing interactive systems. Recent work has shown Extended Reality Prototyping (XRP)'s potential, but its applicability to specific domains like controlling complex machinery needs further exploration. This paper explores the benefits and limitations of XRP in controlling a mobile medical imaging robot. We compare two XR visualization techniques to reduce perceived latency between user input and robot activation. Our XRP validation study demonstrates its potential for comparative studies, but identifies a gap in modeling human behavior in the analytic XRP validation framework.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tex/00_0_acronyms.tex <==
\newcommand{\condREAL}{REAL}
\newcommand{\condMED}{MED}
\newcommand{\condXRP}{XRP}
\newcommand{\condDIR}{DIR}
\newcommand{\condSTE}{STE}
\newcommand{\condSUR}{SUR}

\acrodef{XR}[XR]{Extended Reality}
\acrodef{AR}[AR]{Augmented Reality}
\acrodef{VR}[VR]{Virtual Reality}
\acrodef{MR}[MR]{Mixed Reality}
\acrodef{OST}[OST]{optical see-through}
\acrodef{VST}[VST]{video see-through}
\acrodef{HMD}[HMD]{head-mounted display}
\acrodef{IBR}[IBR]{image-based rendering}
\acrodef{TCT}[TCT]{Task Completion Time}
\acrodef{SEQ}[SEQ]{Single Ease Question}
\acrodef{SUS}[SUS]{System Usability Scale}
\acrodef{XRP}[XRP]{Extended Reality Prototyping}
% \acrodef{UX}[UX]{user experience}
\acrodef{TCT}[TCT]{task completion time}
\acrodef{CBCT}[CBCT]{cone-beam computer tomography}
\acrodef{SoA}[SoA]{Sense of Agency}

==> tex/00_0_commands.tex <==
\newcommand{\ie}{i.e.,}
\newcommand{\eg}{e.g.,}
\newcommand{\etal}{et~al.}
\newcommand{\etc}{etc.}
\newcommand{\chisq}[3]{$\chi^2$(#1)$=$#2,p$=$#3}
\newcommand{\wilc}[3]{Z$=$#1,p#2,r$=$#3}
\newcommand{\chisqtext}[3]{~(\chisq{#1}{#2}{#3})}
\newcommand{\wilctext}[3]{~(\wilc{#1}{#2}{#3})}
\newcommand{\art}[4]{$F$(#1,#2)$=$#3,p#4}
\newcommand{\artcon}[4]{t(#1)$=$#2,p#3,d=#4}
\newcommand{\arttext}[4]{~(\art{#1}{#2}{#3}{#4})}
\newcommand{\artcontext}[4]{~(\artcon{#1}{#2}{#3}{#4})}
%\newcommand{\data}[3]{#1 (#2), #3}
\newcommand{\data}[3]{#1 (#2), #3}
\newcommand{\datatable}[3]{#1 & #2 & #3}

==> tex/00_0_custom_packages.tex <==
\usepackage{tabularx}
\usepackage[table,svgnames]{xcolor}

\usepackage{acronym}
\usepackage{balance}

% set frame for colorbox to enclose text tightly
\setlength{\fboxsep}{1pt}

\usepackage{multirow}

% Strike-through text with \sout{} or \xout{}
\usepackage[normalem]{ulem}

\usepackage{dblfloatfix}

==> tex/00_0_editing_commands.tex <==
% \newcommand{\todoblock}[1]{\textcolor{red}{\textbf{TODO:} \vspace{#1 cm}}}
% \newcommand{\todo}[1]{\textcolor{red}{\textbf{TODO:} #1}}
% \newcommand{\changed}[2]{\textcolor{blue}{#2} \textcolor{red}{(\sout{#1})}}
% \newcommand{\added}[1]{\textcolor{blue}{#1}}
% \newcommand{\deleted}[1]{\textcolor{red}{\sout{#1}}}
% \newcommand{\review}[1]{\textcolor{red}{\textcolor{blue}{#1}}}
% \newcommand{\update}[1]{\textcolor{red}{\textbf{Update:}\textcolor{blue}{#1}}}
% \newcommand{\note}[1]{\marginpar{\small{\textcolor{blue}{#1}}}}
% \newcommand{\revision}[1]{\hl{#1}} % for highlighted camera-ready

%%%%% remove striked out text %%%%
% \renewcommand{\todoblock}[1]{\textcolor{red}{\textbf{TODO:} \vspace{#1 cm}}}
% \renewcommand{\todo}[0]{}
% \renewcommand{\changed}[2]{\textcolor{blue}{#2}}
% \renewcommand{\added}[1]{\textcolor{blue}{#1}}
% \renewcommand{\deleted}[1]{\textcolor{red}{}}
% \renewcommand{\review}[1]{\textcolor{red}{\textcolor{blue}{#1}}}
% \renewcommand{\update}[1]{\textcolor{red}{\textbf{Update:}\textcolor{blue}{#1}}}
% \renewcommand{\note}[1]{\marginpar{\small{\textcolor{blue}{#1}}}}
% \renewcommand{\revision}[1]{\hl{#1}} % for highlighted camera-ready
%%%% END remove striked out text %%%%

%%%% remove all highlights %%%%
% \renewcommand{\todoblock}[1]{\textcolor{red}{\textbf{TODO:} \vspace{#1 cm}}}
% \renewcommand{\todo}[0]{}
% \renewcommand{\changed}[2]{{#2}}
% \renewcommand{\added}[1]{{#1}}
% \renewcommand{\deleted}[1]{\textcolor{red}{}}
% \renewcommand{\review}[1]{\textcolor{red}{\textcolor{blue}{#1}}}
% \renewcommand{\update}[1]{\textcolor{red}{\textbf{Update:}\textcolor{blue}{#1}}}
% \renewcommand{\note}[1]{\marginpar{\small{\textcolor{blue}{#1}}}}
% \renewcommand{\revision}[1]{\hl{#1}} % for highlighted camera-ready
%%%% END remove all highlights%%%%

% \newcommand{\todoky}[1]{\textcolor{red}{\textbf{TODO \textcolor{cyan}{Kevin}:} #1}}
% \newcommand{\todomt}[1]{\textcolor{red}{\textbf{TODO \textcolor{teal}{Markus}:} #1}}
% \newcommand{\todojhp}[1]{\textcolor{red}{\textbf{TODO \textcolor{lime}{JHP}:} #1}}

% \newcommand{\rebuttal}[2]{\textcolor{cyan}{#1 (\textcolor{teal}{#2})}}
% \newcommand{\rebuttalcameraready}[2]{#1}
% \newcommand{\rb}[2]{\rebuttalcameraready{#1}{#2}}
% \newcommand{\rebuttalcamerareadyso}[2]{}
% \newcommand{\rbso}[2]{\rebuttalcamerareadyso{\sout{#1}}{#2}}

==> tex/rebuttal.tex <==
We thank the reviewers for their constructive feedback and appreciate the positive comments about the paper's quality, structure, methodological approach, execution, and writing style, as well as them highlighting interesting and relevant learnings of the paper. In our answers, we address individual reviewers as R1, R2 and R3 and provide a short form summary of each reviewer comment. 

R1 and R3, framework usage: We agree that our evaluation strongly relies on the prototyping framework proposed in related work [48]. To improve the clarity of related methods, we will include a brief overview of their proposed framework in a new subsection of the related work. Furthermore, in this new subsection, we will include additional related frameworks to provide more context and reasoning for the importance of such frameworks (e.g., interaction fidelity framework by McMahan et al.).

R1, specific task: The surgery theater as use case is indeed very specific and the utilized robot is indeed capable of performing very specific medical tasks, namely acquiring cone beam CT images. However, we do not use imaging as a task, but only the general functionality of steering the robot, which can be performed in any scenario. The controls are standard joystick controls similar to a game pad. An important reason for choosing such a sophisticated and specific robot was to provide participants with a meaningful task in a realistic setting and potentially provoke a sense of risk in participants when steering the robot in order to identify differences between REAL and XRP conditions. We believe that the robot and the task are representative of other self-driving and human-steered robots typically used in literature, and that the gathered results are generalizable to other shapes of robots. We will expand the discussion of the transferability of our findings.

R1 and R3, contribution: Using XR for prototyping novel user experiences is an established tool in research and product development, and many research papers rely on XR prototyping to demonstrate the feasibility of novel experiences (as outlined in our related work section). However, there is little research that performs structured validations of XR prototyping to establish the transferability of results to a real use case, i.e., the ecological validity of XR prototyping has not been thoroughly established. Hence, we believe, that insights into validating XR prototyping as a method, i.e., clearly demonstrating relative validity of objective performance measures, is an important contribution to the field. Furthermore, our extensive validation study not only provides novel insights into XR prototyping, but also provides insights into potentially making human-robot interaction more effective. We will add a paragraph at the end of the introduction, to better highlight our contribution compared to the state-of-the-art. 

R3, outliers in TCT, inconsistent ranking SUR in REAL: We expand our discussion regarding outliers in Fig. 3 and the inconsistency in ranking in Fig. 4, both of which are related. As outlined in the discussion ("H2" and "Human Behavior in XRP Framework"), some participants in the SUR condition were not satisfied with relinquishing control to the robot, or worried that the self-driving robot following the ghost would collide with the environment. To compensate for the lack of control, participants developed the strategy to wait for the real robot to catch up with the surrogate visualization. This explains 5/7 TCT outliers in Fig. 3 (Left), 6/8 outliers in Fig. 3 (Middle). 2/7 and 2/8 outliers come from a participant who was generally slower with the surrogate. Despite being slow with SUR, only one of these participants ranked SUR in third place for REAL, and only two participants mentioned insecurities when steering the robot. Apparently, participants who adapted their strategy and slowed down the robot may have had reduced perceived risk during the task, which may have had a positive impact on the ranking. However, other participants (who did not produce outliers) reported insecurities when steering the robot in SUR in the REAL condition due to its higher level of autonomy without adapting their steering strategy, and, thus, ranked SUR in third place. Hence, we will expand our discussion to include this in-depth analysis of the data and the implications on trust when interacting with robots (see paragraph "Delegating Control requires Trust").

R2, sense of agency: We thank R2 for pointing out this concept. We will integrate sense of agency when interacting with machines/robots into our discussion (paragraph "Delegating Control requires Trust") and explore the concept in our future research efforts. Sense of agency or the concept of trust in the human-robot interaction may have been very relevant confounding factors when comparing REAL and XRP in our study, which requires further research to improve the concept of XR prototyping of user experiences.

R1 and R2, participant sample: We agree that in this study, our participant sample is consistent in terms of XR and robot experience so that follow-up studies are warranted. Differences in participant characteristics, such as expertise with robot systems or XR experience, potentially are an important influence in XR validation studies. In this study, we aimed at avoiding bias from extensive prior knowledge of robot systems, which revealed interesting differences between participants in REAL and XRP conditions, such as adapting their steering strategies for SUR, or ranking the SUR condition lower in REAL. Expert users may not have issues with trust in the REAL robotic system as our current inexperienced participants. While, in the discussion, we already mention expertise with robot systems as potential influence on the outcome of a validation study, we will expand this discussion with additional factors relevant for further research. 

R3, interpretation of SUS: We provide the visualization of individual items as an overview to potentially identify issues with one of the conditions. We will remove reporting of individual SUS items in the paper (plots and inferential statistics), and move SUS items to supplemental material to keep the overview of the data. As the individual SUS items were not statistically significant, this will not affect the contribution of the paper. 

R3, robot responsiveness in simulated task environment: The timings of the real robot were replicated faithfully in the simulated robot and consists of three parts. (1) translation speed of the ring at 10cm/second, (2) wheel rotation speed, to align the wheel with a new driving direction, at 22 degrees/second and (3) rotating the ring around its center at a speed of 7.5 degrees/second. We will clarify the speeds of the different components in the paper by streamlining the information in section 3.1 and 3.2, as well as 4.2 when discussing functional fidelity. 

Additionally, for the camera ready version, we will include reviewer suggestions to further improve the writing style, organization and presentation of the paper, e.g. rework the tables (R2, R3), rewrite the caption of Fig. 1 (R3), refine the plots (R3) and make plot referencing more consistent (R3), move superfluous data to the supplemental material and polish the accompanying video.

==> tex/tables/descriptive_fidelity_statistics.tex <==
\begin{table*}[!t]
    \scriptsize
    \begin{tabularx}{\textwidth}{l||X|X|X||X|X|X}
        & \multicolumn{3}{c||}{\condREAL{}} & \multicolumn{3}{c}{\condXRP{}} \\
        \hline
        & \condDIR{} & \condSTE{} & \condSUR{} & \condDIR{} & \condSTE{} & \condSUR{} \\    
        \hline
        \hline
        TCT & \data{135.25}{47.72}{115.0} & \data{133.06}{31.08}{131.8} & \data{86.25}{89.72}{46.6} & \data{111.33}{31.83}{108.6} & \data{112.54}{30.18}{115.9} & \data{66.85}{40.04}{49.5} \\ 
        \hline
        \hline
        Frequency & \data{3.75}{1.03}{4.0} & \data{4.04}{1.00}{4.0} & \data{3.79}{1.18}{4.0} & \data{3.75}{1.03}{4.0} & \data{3.83}{0.92}{4.0} & \data{3.75}{1.15}{4.0} \\

        Complexity & \data{2.00}{1.10}{2.0} & \data{1.88}{1.12}{2.0} & \data{1.88}{1.23}{1.0} & \data{1.92}{1.02}{2.0} & \data{1.50}{0.93}{1.0} & \data{2.08}{1.35}{1.5} \\
        
        Ease of Use & \data{4.00}{0.93}{4.0} & \data{4.38}{0.58}{4.0} & \data{4.21}{0.88}{4.0} & \data{4.08}{1.06}{4.0} & \data{4.58}{0.50}{5.0} & \data{4.12}{1.33}{5.0} \\
        
        Technical Help & \data{1.58}{0.88}{1.0} & \data{1.50}{0.66}{1.0} & \data{1.54}{0.83}{1.0} & \data{1.46}{0.83}{1.0} & \data{1.25}{0.53}{1.0} & \data{1.33}{0.70}{1.0} \\
        
        Function Integration & \data{4.21}{0.88}{4.0} & \data{4.08}{0.93}{4.0} & \data{4.17}{0.87}{4.0} & \data{4.04}{0.86}{4.0} & \data{4.46}{0.66}{5.0} & \data{4.04}{1.23}{4.5} \\
        
        Inconsistency & \data{1.62}{0.88}{1.0} & \data{1.88}{1.19}{1.0} & \data{1.88}{1.12}{2.0} & \data{1.83}{0.96}{2.0} & \data{1.67}{0.82}{1.5} & \data{1.54}{0.88}{1.0} \\
        
        Quick Learning & \data{4.12}{0.99}{4.0} & \data{4.46}{0.59}{4.5} & \data{4.33}{0.64}{4.0} & \data{4.38}{0.77}{4.5} & \data{4.58}{0.50}{5.0} & \data{4.33}{0.96}{5.0} \\
        
        Cumbersome & \data{2.17}{1.09}{2.0} & \data{1.88}{1.08}{2.0} & \data{2.00}{1.25}{1.5} & \data{2.04}{1.00}{2.0} & \data{1.75}{1.03}{1.0} & \data{2.04}{1.33}{1.0} \\
        
        Confidence & \data{4.21}{0.88}{4.0} & \data{4.29}{0.69}{4.0} & \data{3.88}{1.26}{4.0} & \data{4.21}{0.83}{4.0} & \data{4.58}{0.58}{5.0} & \data{4.25}{0.94}{4.5} \\
        
        Required Learning & \data{1.42}{0.58}{1.0} & \data{1.46}{0.72}{1.0} & \data{1.54}{0.93}{1.0} & \data{1.46}{0.59}{1.0} & \data{1.25}{0.44}{1.0} & \data{1.38}{0.71}{1.0} \\

        \hline\hline
        
        Mental Demand & \data{7.00}{4.70}{5.0} & \data{6.88}{4.26}{6.0} & \data{6.58}{5.07}{5.5} & \data{5.79}{4.83}{3.5} & \data{4.54}{4.46}{3.0} & \data{5.58}{4.61}{4.0} \\

        Physical Demand & \data{6.46}{5.18}{4.0} & \data{6.33}{5.43}{4.0} & \data{5.04}{4.87}{2.5} & \data{5.17}{4.22}{4.5} & \data{4.67}{4.46}{3.0} & \data{4.96}{4.71}{2.0} \\
        
        Task Pace & \data{3.83}{3.41}{3.0} & \data{4.25}{3.85}{3.0} & \data{3.96}{3.75}{2.0} & \data{3.75}{3.79}{2.0} & \data{3.71}{3.59}{3.0} & \data{4.21}{3.73}{2.0} \\
        
        Success & \data{5.04}{4.75}{3.0} & \data{3.67}{3.60}{3.0} & \data{5.42}{4.45}{3.0} & \data{4.04}{3.54}{3.0} & \data{3.29}{3.44}{2.5} & \data{2.67}{1.55}{2.0} \\
        
        Commitment & \data{6.71}{4.61}{5.5} & \data{5.71}{4.03}{4.0} & \data{5.75}{4.52}{4.0} & \data{5.04}{4.27}{4.0} & \data{3.96}{3.28}{3.0} & \data{4.42}{3.74}{3.0} \\
        
        Stress & \data{6.00}{4.13}{5.0} & \data{4.46}{3.55}{3.5} & \data{5.67}{4.37}{4.0} & \data{5.29}{3.87}{4.5} & \data{3.08}{3.01}{3.0} & \data{3.71}{4.04}{2.0} \\

        \hline\hline
        
        Usability & \data{78.75}{15.97}{80.0} & \data{81.67}{12.28}{82.5} & \data{78.85}{19.01}{82.5} & \data{79.38}{15.06}{80.0} & \data{86.56}{10.60}{88.8} & \data{80.31}{19.59}{85.0} \\
        
        Task Load & \data{29.20}{18.18}{24.2} & \data{26.08}{15.45}{20.4} & \data{27.01}{18.16}{21.2} & \data{24.24}{15.08}{22.5} & \data{19.38}{14.30}{16.2} & \data{21.28}{14.69}{15.0} \\
    \end{tabularx}    
    \caption{Dependent variable outcomes (mean, std. dev., median) for each individual Realism and Visualization combination.}
    \label{tab:descriptive_fidelity_statistics}
\end{table*}

==> tex/tables/descriptive_statistics.tex <==
\begin{table*}[!t]
   \scriptsize
     \begin{tabularx}{\textwidth}{l||X|X|X||X|X}
        & \condDIR{} & \condSTE{} & \condSUR{} & \condREAL{} & \condXRP{} \\    
        \hline
        \hline
        TCT & \data{123.29}{41.91}{112.3} & \data{122.80}{32.03}{119.8} & \data{76.55}{69.42}{47.8} & \data{118.19}{64.62}{112.0} & \data{96.91}{40.01}{94.3} \\
        \hline
        \hline
        Frequency & \data{3.75}{1.02}{4.0} & \data{3.94}{0.95}{4.0} & \data{3.77}{1.15}{4.0} & \data{3.86}{1.07}{4.0} & \data{3.78}{1.02}{4.0} \\

        Complexity & \data{1.96}{1.05}{2.0} & \data{1.69}{1.03}{1.0} & \data{1.98}{1.28}{1.0} & \data{1.92}{1.14}{2.0} & \data{1.83}{1.13}{1.0} \\
        
        Ease of Use & \data{4.04}{0.99}{4.0} & \data{4.48}{0.55}{4.5} & \data{4.17}{1.12}{5.0} & \data{4.19}{0.82}{4.0} & \data{4.26}{1.03}{5.0} \\
        
        Technical Help & \data{1.52}{0.85}{1.0} & \data{1.38}{0.61}{1.0} & \data{1.44}{0.77}{1.0} & \data{1.54}{0.79}{1.0} & \data{1.35}{0.70}{1.0} \\
        
        Function Integration & \data{4.12}{0.87}{4.0} & \data{4.27}{0.82}{4.0} & \data{4.10}{1.06}{4.0} & \data{4.15}{0.88}{4.0} & \data{4.18}{0.95}{4.0} \\
        
        Inconsistency & \data{1.73}{0.92}{1.0} & \data{1.77}{1.02}{1.0} & \data{1.71}{1.01}{1.0} & \data{1.79}{1.06}{1.0} & \data{1.68}{0.89}{1.0} \\
        
        Quick Learning & \data{4.25}{0.89}{4.0} & \data{4.52}{0.55}{5.0} & \data{4.33}{0.81}{4.5} & \data{4.31}{0.76}{4.0} & \data{4.43}{0.77}{5.0} \\
        
        Cumbersome & \data{2.10}{1.04}{2.0} & \data{1.81}{1.04}{1.5} & \data{2.02}{1.28}{1.0} & \data{2.01}{1.13}{2.0} & \data{1.94}{1.12}{2.0} \\
        
        Confidence & \data{4.21}{0.85}{4.0} & \data{4.44}{0.65}{5.0} & \data{4.06}{1.12}{4.0} & \data{4.12}{0.98}{4.0} & \data{4.35}{0.81}{5.0} \\
        
        Required Learning & \data{1.44}{0.58}{1.0} & \data{1.35}{0.60}{1.0} & \data{1.46}{0.82}{1.0} & \data{1.47}{0.75}{1.0} & \data{1.36}{0.59}{1.0} \\
        \hline
        \hline
        
        Mental Demand & \data{6.40}{4.75}{4.0} & \data{5.71}{4.47}{4.0} & \data{6.08}{4.82}{4.5} & \data{6.82}{4.62}{5.0} & \data{5.31}{4.60}{3.5} \\

        Physical Demand & \data{5.81}{4.72}{4.0} & \data{5.50}{4.99}{3.0} & \data{5.00}{4.74}{2.0} & \data{5.94}{5.13}{3.5} & \data{4.93}{4.41}{3.0} \\
        
        Task Pace & \data{3.79}{3.57}{3.0} & \data{3.98}{3.69}{3.0} & \data{4.08}{3.70}{2.0} & \data{4.01}{3.63}{3.0} & \data{3.89}{3.66}{2.0} \\
        
        Success & \data{4.54}{4.18}{3.0} & \data{3.48}{3.49}{3.0} & \data{4.04}{3.58}{3.0} & \data{4.71}{4.30}{3.0} & \data{3.33}{3.00}{3.0} \\
        
        Commitment & \data{5.88}{4.48}{4.5} & \data{4.83}{3.74}{3.5} & \data{5.08}{4.16}{3.0} & \data{6.06}{4.36}{4.0} & \data{4.47}{3.76}{3.0} \\
        
        Stress & \data{5.65}{3.98}{5.0} & \data{3.77}{3.33}{3.0} & \data{4.69}{4.28}{3.0} & \data{5.38}{4.03}{4.0} & \data{4.03}{3.73}{3.0} \\
        \hline
        \hline
    
        Usability & \data{79.06}{15.36}{80.0} & \data{84.11}{11.62}{82.5} & \data{79.58}{19.11}{82.5} & \data{79.76}{15.82}{82.5} & \data{82.08}{15.64}{82.5} \\
    
        Task Load & \data{26.72}{16.71}{23.8} & \data{22.73}{15.11}{17.1} & \data{24.15}{16.60}{18.8} & \data{27.43}{17.11}{21.2} & \data{21.63}{14.63}{16.7} \\
    \end{tabularx}    
    \caption{Dependent variable outcomes (mean, std. dev., median) for each overall Realism and Visualization.}
    \label{tab:descriptive_statistics}
\end{table*}
